The Road to Trust: Building Enclaves within Confidential VMs

Integrity is critical for maintaining system security, as it ensures that only genuine software is loaded onto a machine. Although confidential virtual machines (CVMs) function within isolated environments separate from the host, it is important to recognize that users still encounter challenges in maintaining control over the integrity of the code running within the trusted execution environments (TEEs). The presence of a sophisticated operating system (OS) raises the possibility of dynamically creating and executing any code, making user applications within TEEs vulnerable to interference or tampering if the guest OS is compromised. To address this issue, this paper introduces NestedSGX, a framework which leverages virtual machine privilege level (VMPL), a recent hardware feature available on AMD SEV-SNP to enable the creation of hardware enclaves within the guest VM. Similar to Intel SGX, NestedSGX considers the guest OS untrusted for loading potentially malicious code. It ensures that only trusted and measured code executed within the enclave can be remotely attested. To seamlessly protect existing applications, NestedSGX aims for compatibility with Intel SGX by simulating SGX leaf functions. We have also ported the SGX SDK and the Occlum library OS to NestedSGX, enabling the use of existing SGX toolchains and applications in the system. Performance evaluations show that context switches in NestedSGX take about 32,000 -- 34,000 cycles, approximately $1.9\times$ -- $2.1\times$ higher than that of Intel SGX. NestedSGX incurs minimal overhead in most real-world applications, with an average overhead below 2% for computation and memory intensive workloads and below 15.68% for I/O intensive workloads.

==> tex/design_backup.tex <==
\section{Design}
\label{sec:design}
%This section introduces the design of \sysname. We begin with an overview of the major components, followed by the memory isolation scheme and enclave life cycle management. Finally, we delve into how the enclave is measured and attested.

\subsection{Overview}
\label{subsec:overview}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figs/overview2.pdf}
    \caption{\sysname overview. The security monitor, the SGX emulation layer and the enclave operate in the kernel and user mode at VMPL0, while the guest OS and App operate in the kernel and user mode at VMPL1. The transitions between VMPL0 and VMPL1 occur via the untrusted host.}
    \label{fig:overview}
\end{figure}

\revision{outlines the principles or insights used in NestedSGX.}

As shown in Fig.~\ref{fig:overview}, \sysname encompasses the following components within the CVM. 
%\begin{packeditemize}
%  \item 
The application is divided into the trusted part (\textit{\textbf{enclave}}) and the untrusted part (\textit{\textbf{App}}). 
%\item  
The \textit{\textbf{security monitor}} is responsible for enforcing security isolation within \sysname.
%and runs at the highest privileged VMPL (i.e., VMPL0). 
The \textit{\textbf{SGX emulation layer}} emulates SGX instructions, and serves as the root of trust (RoT) for measurement and reporting of the enclave.
%It 
%  \item 
The \textit{\textbf{guest OS}}
%(such as popular Linux distributions) 
offers essential features to applications, such as file systems, networking, device drivers, and language runtime.
%\end{packeditemize}
%The security monitor and the enclave operates in the kernel and user mode at VMPL0, while the guest OS and App operates in the kernel and user mode at VMPL1. 这句不要了，secondly里有这一句



To enforce memory isolation, the security monitor runs at the highest privileged VMPL (i.e., VMPL0). On the other hand,
%Due to the need for accessing both the address spaces of the guest OS and the enclave when emulating certain SGX instructions (such as EADD), the  SGX emulation layer runs at a higher privileged VMPL than the guest OS and App. 
%It is important to note that
we cannot place the SGX emulation layer in a VMPL lower than that of the guest OS (e.g., guest OS in VMPL1 and SGX emulation layer in VMPL2). Doing so would grant the guest OS the ability to generate attestation reports on behalf of the SGX emulation layer, potentially compromising the trust chain (please refer to Sec.~\ref{subsec:attestation} for details).
%the enclave operate at higher privileged VMPLs, 
Within our threat model, we consider the SGX emulation layer to be trusted. 
%For brevity, in the rest of the paper we 
%Currently, we have made the decision to 
%consider \textit{the SGX emulation layer as part of the
%run both the 
%security monitor}, both running at VMPL0,
For the sake of brevity, throughout the remainder of the paper, we regard \textit{the SGX emulation layer as an integral component of the security monitor}, both running at VMPL0.
while the guest OS and App operate at a lower privileged VMPL (i.e., VMPL1). 
Within this design, we also place the enclaves within the same VMPL as the SGX emulation layer, in the user mode and kernel mode respectively, since if they were placed at different VMPLs, a context switch between the enclave and App would necessitate 2 costly VMPL switches.
%One such example is the EADD instruction, which involves copying the content of a memory page from the application to the enclave.Therefore, it is more reasonable to position the SGX emulation layer in VMPL0, as it has access to both address spaces.
In practice, however, if running both the SGX emulation layer and the enclaves in VMPL0 raises security concerns, we can adapt NestedSGX slightly as follows: the security monitor still runs in VMPL0; the SGX emulation layer and the enclaves run in the kernel and user mode at VMPL1, and the guest OS and the App run in the lowest VMPL (e.g., VMPL3).

%current privilege level 0 (CPL0) in VMPL1, and the enclaves run at CPL3 in VMPL1; the guest OS runs in the lowest VMPL (e.g., VMPL3).

To let the users maintain control over the code running inside the CVM and bootstrap trust to the enclave within a feature-rich guest OS, \sysname is designed to fulfill the following requirements. 

\textit{Firstly}, \sysname ensures that any transitions between the trusted and untrusted components are mediated by the security monitor. This guarantees that sensitive information is properly sanitized and safeguarded. To leverage existing SGX toolchains, \sysname employs the SGX programming model to manage the enclave's life cycle.
The details for secure enclave state transitions will be presented in Sec.~\ref{subsec:transitions}.

\textit{Secondly}, the system establishes isolated memory regions exclusively used by the security monitor, the enclaves and the guest OS respectively. This ensures that the enclave and the security monitor are secure even in scenarios where the guest OS operates in kernel mode. Specifically, the entire gPA space is divided to two parts: a continuous and fixed region exclusively used by VMPL0, and the remaining portion used by VMPL1. 
Additionally, our design guarantees that the enclave cannot access the memory of the guest OS, despite running at a higher VMPL.
The details of the memory isolation scheme will be presented in Sec.~\ref{subsec:isolation}.


\textit{Lastly}, in \sysname, only authenticated code and data can be loaded and processed within the enclave. 
%The integrity of the enclave is measured and can be attested to ensure its trustworthiness. 
To achieve this, \sysname enforces a mechanism where the enclave can only be loaded by the trusted security monitor, which also performs the measurement of the enclave's integrity.
While the guest OS retains the freedom to load and execute any code within its own address space, these code segments are not affirmed by the security monitor and therefore will not be attested.
The details of enclave measurement and attestation will be presented in Sec.~\ref{subsec:attestation}.


%With this adapted design, we can provide the SGX emulation layer with complete access to the guest OS's address space while reusing the NestedSGX design.


\begin{table*}
    \centering
    \caption{Comparison with competing approaches.}
    \label{tab:comparison}
    %\small{
    \begin{tabular}{c C{2.0cm} C{2.0cm}  C{2.0cm}  C{2.0cm} C{2.0cm} C{2.0cm}}
    %\begin{tabular}{c c c c c c c}
    \toprule
         & \textbf{Unlimited enclaves} & \textbf{Multi-threading} & \textbf{Exception handling} & \textbf{SGX ecosystem} & \textbf{No changes to hypervisor} & \textbf{Low-overhead context switches}  \\ \midrule
        vSGX~\cite{zhao2022vsgx} & \XSolidBrush & \Checkmark & \Checkmark  & \Checkmark  & \XSolidBrush & \XSolidBrush \\ \midrule
        Veil~\cite{ahmad2023veil} & \Checkmark  & \XSolidBrush & \XSolidBrush & \XSolidBrush & \XSolidBrush & \Checkmark  \\ \midrule
        \sysname & \Checkmark  & \Checkmark  & \Checkmark  & \Checkmark & \Checkmark & \Checkmark \\ \bottomrule
    \end{tabular}
    %}
\end{table*}

\para{Comparison with competing approaches (Table~\ref{tab:comparison})}
%\wenhao{Veil}
%\para{Comparison with vSGX~\cite{zhao2022vsgx}}
%\wenhao{this subsection needs to be revised}
vSGX~\cite{zhao2022vsgx} effectively virtualizes Intel SGX on AMD SEV, ensuring complete binary compatibility and the execution of unmodified SGX programs. vSGX employs two separated CVMs to accommodate the untrusted application and the enclave. In contrast, \sysname adopts a more intuitive design that utilizes different VMPLs for memory isolation. The \sysname design offers the following benefits.

Firstly, vSGX cannot support directly sharing encrypted memory between the enclave VM (EVM) and application VM (AVM). To provide confidentiality, integrity and replay protection, a dedicated communication protocol and encrypted channel are essential. Within \sysname, the security monitor can access the entire guest physical address space, and communicate with the guest OS through shared memory. This approach circumvents the overhead associated with memory encryption and movement, and prevents the hypervisor from observing traffic patterns. As a comparison, an empty ECALL costs 1.5 ms on vSGX, and only 12 us on \sysname, which is two orders of magnitude faster than vSGX.

Secondly, with vSGX, only one enclave can be hosted within the EVM, which restricts the maximum number of concurrently-running enclaves on the hardware platform. This limitation arises because SEV associates ASIDs with VMs' memory encryption keys, and the ASID bit is limited. In contrast, \sysname has the ability to support an unlimited number of enclaves.

More importantly, \sysname does not serve as a direct substitute for vSGX. On vSGX, the enclave thread and application thread operate with different vCPUs in separated VMs. Specifically, the application thread at the AVM is paused on EENTER; upon receiving the EENTER request, the EVM creates a thread to handle it in the EVM. On \sysname, the enclave thread and application thread operate with the same vCPU, while the vCPU contexts associated with different VMPLs are saved in different VMSAs. Consequently, managing the entry and exit of enclaves on \sysname necessitates meticulous handling of vCPU state transitions. As an evidence, AEX is relatively straightforward on vSGX: vSGX simply puts the enclave thread to sleep on AEX, then wakes it and resumes the execution directly on ERESUME. On \sysname the enclave context needs to be saved on AEX and recovered on ERESUME.

Concurrent to our work, 
%Very recently, 
Ahmad et al. proposed Veil~\cite{ahmad2023veil} as a service framework running at VMPL0 (presented at ASPLOS 2024). 
%The concept of Veil is quite similar to AMD's Secure VM Service Module (SVSM). 
As one use case, Veil offers protection to the entire applications within a separated VMPL, facilitating redirection of system calls and interrupts. However, unlike our approach, it does not focus on protecting a trusted portion of the application or strive for compatibility with Intel SGX. Currently, Veil lacks support for multi-threading and exception handling. In contrast, \sysname leverages an existing SGX toolchain by emulating most SGX instructions, thereby naturally providing support for multi-threading and exception handling.

\revision{Addressing these limitations requires an SGX emulation layer to emulate SGX instructions and fulfill certain OS functionalities, such as mediating all enclave-App context switches and forwarding exceptions to the guest OS, within the user-land enclave’s VMPL. Designing and implementing this layer is challenging because its state—including general-purpose and segment registers, stack pointers—changes during context switches when handling various requests (e.g., forwarding exceptions or emulating SGX instructions), so when the system re-enters the enclave again, its state cannot be fully restored due to the change of the state in the emulation layer that handles the context switch. As a result, the handling of subsequent requests can lead to failures, such as faults and stack exhaustion.}

\revision{Note that this challenge cannot be resolved by vSGX or Veil. vSGX runs the App and enclave in different VMs and can simply pause or activate one of them for context switching, but also incurs significant overheads for cross-VM communications during the switch. Context switches in Veil rely on hardware, which automatically saves and restores the contexts of the enclave and the guest OS within their respective VMSAs. But this mechanism cannot handle the switches triggered by exceptions.}

\revision{Our solution introduces a unique design that models the states of the SGX emulation layer using a finite state machine (FSM). After each context switch, the layer restores its original state under the FSM's guidance. We achieve this by pairing asynchronous and synchronous enclave entry and exit requests. We save the state of the SGX emulation layer before the entry request (eenter/AEX) and restore it after processing the exit request, through a carefully designed restoration strategy based upon the FSM (e.g., restoring gs before rsp to balance the stack). In this way, the enclave state can be guaranteed to be correct no matter how complicated the request sequence could become (e.g., arbitrary exceptions between eenter and eexit). This design, along with our thorough implementation of exception handling and multithreading, differentiates NestedSGX from both Veil and vSGX.}

\subsection{Enclave life cycle management}
\label{subsec:transitions}

In \sysname, the life cycle of an enclave closely resembles that of SGX. Initially, the application invokes the ECREATE leaf function to create the enclave, which initializes the SGX Enclave Control Structure (SECS) page. Subsequently, EPC pages necessary for the enclave, such as code sections, data sections, and Thread Control Structure (TCS) pages, are added using EADD and measured using EEXTEND leaf functions.
Once all the required EPC pages are added, the enclave is initialized with EINIT, and the final measurement is performed. Upon completion of the enclave's execution, the EPC pages are reclaimed using the EREMOVE leaf function, and the enclave is destroyed.

\sysname achieves compatibility with Intel SGX by transitioning to the security monitor on these leaf functions. Since VMPL switches can only be executed in the privileged mode (Sec.~\ref{subsec:snp}), \sysname provides the \sysname-driver within the guest OS, which accepts the request from the App and facilitates the VMPL switch. During this process, the \sysname-driver receives the type of SGX leaf functions, while the parameters are saved on the App's stack. The \sysname-driver then switches the execution to VMPL0 and transfers control to the security monitor, where the security monitor emulates the instructions strictly adhering to the SGX specifications.

%For transitioning from the App (VMPL1) to the security monitor (VMPL0), since the instructions for VMPL switches can only be executed in the privileged mode (Sec.~\ref{subsec:snp}), \sysname provides the \sysname-driver within the guest OS, which accepts the request from the App and facilitates the VMPL switch. During this process, the \sysname-driver receives the type of SGX instructions, while the parameters are saved in the marshalling buffer. The \sysname-driver then switches the execution to VMPL0 and transfers control to the security monitor. 


%accepts the request from the App and conducts the VMPL switch. In this process, the type of SGX instructions is passed to the \sysname-driver, while the parameters are saved on the App's stack. The \sysname-driver switches the execution to VMPL0 and passes control to the security monitor, which emulates the instruction, 


\begin{figure*}
    \centering   
    \includegraphics[width=\linewidth]{figs/lifecycle2.pdf}
    \caption{The management of enclave life cycles, e.g., handling synchronous and asynchronous enclave entry and exit events.}
    \label{fig:lifecycle}
\end{figure*}


\para{Synchronous enclave entry and exit}
Once an enclave is initialized, the App can enter the enclave using the EENTER leaf function and jump to the enclave's code for execution. 
As shown in Fig.~\ref{fig:lifecycle}, during the emulation of EENTER, the security monitor switches to the enclave's page table and enters the enclave entry point specified by the TCS using the \texttt{sysret} instruction. The enclave can then return to the App using the EEXIT leaf function, which is also emulated by the security monitor. Specifically, the enclave returns to the security monitor using the \texttt{syscall} instruction. Subsequently, the security monitor switches the execution to the \sysname-driver running at VMPL1. The \sysname-driver restores the App's page table and returns control to the App using the \texttt{sysret} instruction.

\para{Asynchronous enclave entry and exit}
During enclave execution, faults and exceptions may occur. In accordance with the SGX model, these faults and exceptions are supposed to be handled by the guest OS first.
In \sysname, when a fault or exception occurs within the enclave, it traps to the fault and exception handler within the security monitor (Fig.~\ref{fig:lifecycle}). The security monitor then emulates the Asynchronous Exit (AEX) event by saving the context of the enclave in the state saving area (SSA). Subsequently, the security monitor switches the vCPU to the \sysname-driver, which operates at VMPL1. The \sysname-driver fills the instruction pointer (RIP) to the trampoline area (AEP)
%specified in the TCS 
and invokes the handler of the guest OS. After the OS handles the fault or exception, it uses the \texttt{iret} instruction to return to the AEP. The AEP, in turn, resumes the execution of the enclave using the ERESUME leaf function. 
% The security monitor emulates the ERESUME instruction similar to how it emulates the EENTER instruction, with the distinction that the enclave's execution context is restored from the SSA.
The emulation of the ERESUME leaf function is similar to that of EENTER, except that the enclave's execution context is restored from the SSA.
As a result, \sysname is capable of handling exceptions that occur during enclave execution. For example, \sysname supports the emulation of the CPUID instruction, enabling the execution of unmodified applications.\footnote{In comparison, vSGX~\cite{zhao2022vsgx} requires modifying the application code in order to bypass the CPUID check.}

It's worth noting that if the untrusted \sysname-driver chooses not to fill RIP with AEP, this decision does not introduce any new security issues. This is because the control flow outside the enclave is already vulnerable to manipulation within the SGX model and is not inherently trusted.
In \sysname, faults and exceptions are firstly trapped to the security monitor, enabling easy detection of suspicious behaviors such as abnormal interrupts caused by page fault-based attacks. 
%\link{I guess it might be better to use "Under these circumstances" or "Conceptually" instead of "Additionally", cause as it puts, the implementation about these two features might be futural work, but conceptually these features can be added into the exception handler part in the Rust Monitor. Please don't change this before we have a discussion on it.} 
Conceptually, \sysname can also support the recent AEX-notify feature~\cite{constable2023aex},
% as well as enclave dynamic memory management (EDMM)~\cite{mckeen2016edmm} in SGX, 
although the implementation is planned for future work.


%\wenhao{this also prevents the fault-based attacks, and can support AEX-notify? mention it here, instead of in security analysis section}

\subsection{Memory isolation}
\label{subsec:isolation}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figs/memory2.pdf}
    \caption{The guest physical address space is divided into 3 parts: the secure memory used by the security monitor, the EPC memory, and the normal memory.}
    \label{fig:memory}
\end{figure}

The entire guest physical address space of the CVM is divided into 3 parts (Fig.~\ref{fig:memory}): the secure memory used by the security monitor, the secure memory used by the enclaves (i.e., EPC), and the normal memory used by the guest OS and untrusted applications. The access to the secure memory is restricted solely to VMPL0, whereas the normal memory can be accessed by both VMPL0 and VMPL1. Notably, the SGX control structures are stored in the memory of the security monitor, while the enclave's code and data pages are stored in the memory reserved for the EPC.

\para{Booting \sysname}
Upon receiving a request to launch a CVM, the platform proceeds to load the VM image and cryptographically measures its contents. During the initialization process, the entire gPA is divided into two distinct parts. By configuring the RMP attributes, we establish a dedicated region of guest memory exclusively reserved for VMPL0, while the remaining gPA regions are reserved for VMPL1. The memory for VMPL0 is further divided into two parts, one for the security monitor and one for the enclaves.

Once the guest image is loaded, the hypervisor places the vCPU in VMPL0 mode and transfers control to the security monitor, which is positioned at the predetermined gPA location. The security monitor takes responsibility of initializing the guest CPU, memory, and setting up a page table for execution. It subsequently hands over control to the BIOS code to initiate the booting process of the guest OS. The security monitor advertises its presence and the memory range reserved for VMPL0. This prevents the guest OS from attempting to utilize any memory within that range. Any such attempts would be detected and blocked by the VMPL permission check, leading to RMP faults. In this manner, \sysname ensures that the guest OS cannot access or interfere with the memory of the security monitor or the enclaves.

%\para{Preventing memory mapping attacks}
\para{EPC memory management}
In Intel SGX, the enclave and application share the same page table, and the hardware prevents memory mapping attacks by performing additional security checks during a page table walk, using the EPCM to ensure that the memory mappings are correct. 
Without hardware support, it is necessary to prevent the guest OS from manipulating the mappings of the enclave. \sysname employs a shadow page table scheme: the application's page table is managed by the guest OS, while the enclave’s page table is managed by the security monitor. In situations where the application and enclave need to share memory, such as for parameter passing, \sysname maps the shared memory to both page tables with the same gVA-to-gPA mapping. The mapping of the parameter buffer remains fixed throughout the entire lifetime of the enclave. Consequently, we do not need to maintain the synchronization of the two page tables.

%\wenhao{memory management(free-list?)/allocation/recycling}
%\link{i remember in xv6 implementation, only one list is maintained for the physical memory allocator. But the cost is great..}

In \sysname, the security monitor is responsible for managing the EPC memory. It maintains two lists: a free list and a used list, containing all the EPC pages. Similarly, an EPCM data structure is utilized to track the state of each EPC page. During enclave initialization, when an EPC page needs to be added to the enclave (via EADD), the security monitor selects a page from the free list and constructs the corresponding page table entry (PTE).

% \textcolor{red}{During EADD, the security monitor chooses one page from the free list of all EPC pages, and construct the corresponding PTEs.}

%\wenhao{page swapping and page faults handling}
%\wenhao{@link: please check %\link{checked}}
In cases when the enclave's memory accesses result in a page fault, the CPU triggers a trap to the security monitor. The security monitor forwards the page fault information, including the address of the faulting page, to the \sysname-driver. If the \sysname-driver determines that a page frame needs to be allocated for the enclave, it requests the security monitor to allocate a physical page within the EPC. Additionally, the security monitor constructs the corresponding PTE in the enclave's page table. Once the page fault is successfully handled, the security monitor restores the enclave's execution context.
Currently, \sysname does not support swapping the enclave's pages to regular memory or disk storage.

\ignore{
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figs/pagefault.pdf}
    \caption{Handling Page faults in \sysname.}
    \label{fig:pagefault}
\end{figure}
}

\para{Isolation of enclaves}
% explain why we do not put the enclaves in another VMPL (e.g., VMPL1)
It is also important to prevent an enclave from tampering with the security monitor or the guest OS. This ensures protection against potentially malicious enclave (i.e., enclave malware) or enclaves that may have vulnerabilities that could be exploited.
One approach to address this concern is to place the enclave at a distinct VMPL level, separate from VMPL0 or VMPL1, and enforce the appropriate VMPL permissions to contain the enclave code. However, the transition is mediated by the security monitor, necessitating at least two VMPL switches. As a result, transitioning between the application and the enclave becomes costly.

Instead, the enclave is positioned in user mode at VMPL0 and isolated using traditional page table-based isolation. Specifically, \sysname ensures that the enclave's page table does not map to any gPA belonging to the security monitor or the guest OS. As a result, transition between the application and the enclave only requires one VMPL switch.

%----------------------

%The instructions for enclave creation, EPC memory allocation, deallocation, measurement cannot be misused by user programs and hence are privileged (ENCLS). We introduce a kernel loadable module in guest OS to provide the execution environment for guest privileged state running corresponding hypercall instructions without modifying guestOS. These instructions are again exposed through ioctl() syscall interface to applications residing in guest user mode.



\subsection{Measurement, attestation and sealing}
\label{subsec:attestation}

When the CVM image is loaded and measured, the page attributes, including the access permissions of all VMPLs, are included in the measurement. Any attempts to modify the code and data in VMPL0 and VMPL1, or to manipulate the access permissions of guest pages during CVM initialization, will be reflected in the measurement.
After the CVM is initialized, software operating at any VMPL level can initiate an attestation report request by sending a message to the AMD-SP firmware. The request structure comprises the VMPL level and 512 bits of space for user-provided data, which will be incorporated into the attestation report signed by the AMD hardware. The local/remote attestation and sealing mechanisms of \sysname closely mirror those employed by Intel SGX.
This is accomplished by emulating the corresponding instructions (i.e., EGETKEY and EREPORT) within the security monitor.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figs/attestation2.pdf}
    \caption{The \sysname attestation report consists of two parts: the SEV-SNP attestation report signed by VCEK, and the enclave report signed by \sysname AIK. The \sysname AIK is generated within the security monitor and subsequently bound to the SEV-SNP hardware by placing its public key as part of the SEV-SNP attestation report.}
    \label{fig:attestation}
\end{figure}


\para{Chain of trust}
When the CVM is first initialized, the security monitor randomly generates a key pair, which serves as the attestation identity key (AIK) of \sysname. The AIK is only required to be generated once and can be reused across different CVM boot cycles. To establish the binding between \sysname's AIK and the CVM, we include the digest of the public part of the attestation key in the user-data field of the attestation report request (Fig.~\ref{fig:attestation}), while the private key never leaves the memory of the security monitor.%\wenhao{a figure for key management}

The security monitor initiates the generation of an \textit{SEV-SNP attestation report} by dispatching a SNP\_REPORT\_REQ message to the AMD-SP hardware.
The request message between the security monitor and AMD SP is encrypted using the appropriate VM Platform Communication Key (VMPCK) for VMPL0. 
Upon receiving the encrypted message, the AMD-SP hardware decrypts it, verifies its integrity, and subsequently responds with an attestation report, which is signed with the SEV-SNP attestation key (Versioned Chip Endorsement Key, VCEK). The report includes the platform measurement, the security monitor measurement, the VMPL level, and the public key of \sysname's AIK.
The \sysname AIK is exclusively accessible to the quoting enclave (QE) and is subsequently used to sign the report of the enclave. This signed enclave report, along with the SEV-SNP attestation report, collectively constitutes the final attestation report in \sysname.

Upon receiving the final attestation report, the remote party verifies the certificate chain to ensure that the SEV-SNP attestation report is signed by VCEK. This process confirms that the report originates from an authentic AMD processor, has been executed within a CVM, and that the measurements of both the platform and the security monitor are accurate. Furthermore, he gains confidence that the AIK generated by \sysname is produced and retained within the security monitor. Finally, he verifies that the enclave report, which includes the enclave measurement, is signed with \sysname's AIK, concluding the attestation process.

\para{Sealing}
The security monitor can request keys from the AMD-SP by sending a MSG\_KEY\_REQ message to the AMD-SP. Upon receiving the request, the AMD-SP derives a key for the guest from a root key, which is responded to the security monitor and can be used as a sealing key. The sealing key can then be extended to support sealing of the enclave’s secret, binding the key to the enclave’s measurement. As part of the MSG\_KEY\_REQ message, the security monitor specifies that the derived key is used by VMPL0 and the AMD-SP mixes the VMPL information into the derived key.
Although the guest OS running at VMPL1 can also request keys with the MSG\_KEY\_REQ message, it is not allowed to specify VMPL0 in the message, because the hardware ensures that the specified VMPL is greater than or equal to the current VMPL. Therefore, the guest OS cannot derive the same key as the one derived by the security monitor.

% sec 4.5 https://arxiv.org/pdf/2303.16463.pdf

%\para{Quoting enclave}
